Combining reference-star and angular differential imaging for high-contrast imaging of extended sources

High-contrast imaging (HCI) is a technique designed to observe faint signals near bright sources, such as exoplanets and circumstellar disks. The primary challenge in revealing the faint circumstellar signal near a star is the presence of quasi-static speckles, which can produce patterns on the science images that are as bright, or even brighter, than the signal of interest. Strategies such as angular differential imaging (ADI) or reference-star differential imaging (RDI) aim to provide a means of removing the quasi-static speckles in post-processing. In this paper, we present and discuss the adaptation of state-of-the-art algorithms, initially designed for ADI, to jointly leverage angular and reference-star differential imaging (ARDI) for direct high-contrast imaging of circumstellar disks. Using a collection of high-contrast imaging data sets, we assess the performance of ARDI in comparison to ADI and RDI based on iterative principal component analysis (IPCA). These diverse data sets are acquired under various observing conditions and include the injection of synthetic disk models at various contrast levels. Our results demonstrate that ARDI with IPCA improves the quality of recovered disk images and the sensitivity to planets embedded in disks, compared to ADI or RDI individually. This enhancement is particularly pronounced when dealing with extended sources exhibiting highly ambiguous structures that cannot be accurately retrieved using ADI alone, and when the quality of the reference frames is suboptimal, leading to an underperformance of RDI. We finally apply our method to a sample of real observations of protoplanetary disks taken in star-hopping mode, and propose to revisit the protoplanetary claims associated with these disks.

==> poubelle.tex <==
\begin{figure*}[!ht]
\centering
\begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Images/comp_MWC_SPHERE_26dec.png}
        \caption{MWC~758, 26 dec 2022}
        \label{fig:comp_MWC_SPHERE_26dec}
    \end{subfigure}
     \hfill
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Images/comp_MWC_H3SPHERE.png}
        \caption{TOBEDEFINE}
        \label{fig:comp_MWC_H3SPHERE}
    \end{subfigure}
    \hfill
  \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Images/HD_1632962022-06-11a.png}
        \caption{HD~163296 11 july 2022}
        \label{fig:comp_MWC_NIRC2_cube1}
    \end{subfigure}
    \caption{Reduction of three datasets from the survey of young stars hosting
    protoplanetary disks observation with the star-hopping mode of the SPHERE instrument at the Very Large Telescope, we observed, presented by \citet{Ren23a}.
    The three observation, from top to bottom shows (a) MWC~758, (b) and (c) HD~163296. 
    The dataset were reduced using ARDI strategy with \texttt{mustard} (left) and I-PCA (middle) compare to RDI strategy with I-proj (right). The color scale is arbitrary, but consistent between all plots in relative terms and displayed in a logarithmic scale.}
    \label{fig:testrealdata}
\end{figure*}

\subsection{Tests on real data}

\sj{To be completed accodingly}
We reduced with new algorithms three datasets captured while performing star-hopping that were already published in \citet{Ren23a} while being reduced using the data imputation with sequential non-negative
matrix factorization algorithm (DI-sNMF). All of them were taken in K-band with the infrared dual-band imager and spectrograph (IRDIS) camera of the Spectro-Polarimetric High-contrast Exoplanet REsearch coronographic system of the Very Large Telescope (VLT/SPHERE). We selected the three following dataset :
\begin{enumerate}[(a)]
    \item  High quality dataset of MW~C758 (prog~ID \href{https://archive.eso.org/wdb/wdb/eso/sched_rep_arc/query?progid=106.21HJ.001}{106.21HJ.001 0106.C-0192(A)}) that was very successfully reduced by DI-sNMF. The reductions using ARDI with both \texttt{MUSTARD} and I-PCA exhibit very similar visual results to DI-sNMF results from \citet{Ren23a}, while RDI using PCA based algorithm clearly underperforms in comparison. There is a reduced halo surrounding the disk in the predictions made by \texttt{MUSTARD}, although the overall quality of reconstruction with both ARDI algorithms and RDI with DI-sNMF appears similar and exhibits identical structures. In this particular case, the reference stars obtained through star hopping are of sufficient quality, and the disk is adequately bright relative to the intensity of the speckle pattern, such that the 27° angular diversity does not provide significantly more information. Nevertheless, it is worth noting that, similar to DI-sNMF, the proposed I-PCA-based algorithm neither suffers from self-subtractions to the same extent as RDI with PCA nor experiences over-subtraction and flux invariance issues, as seen in algorithms relying solely on ADI.
    
    
    \item Adversarial dataset of HD 163296 (prog~ID \href{https://archive.eso.org/wdb/wdb/eso/sched_rep_arc/query?progid=106.21HJ.001}{106.21HJ.001 0106.C-0192(A)}) for which no appropriate reference star were found, causing DI-sNMF to fail restored the disk. On top of this, the field of view does not present more than $3\degr$ inhibited to properly rely on angular diversity. 
   
    \item An adversarial observation of HD 163296 circumstellar disk (prog~ID \href{https://archive.eso.org/wdb/wdb/eso/sched_rep_arc/query?progid=106.21HJ.001}{106.21HJ.001 0106.C-0192(A)}), which despite being very bright compared to speckle intensity, is quite complicated because not only are the reference stars inappropriate, but there is also very little rotation (only few degrees), so the angular diversity does not provide much information. Our strategy to improve the results using I-PCA is to concatenate numerous reference images to the original dataset and then use a high number of components. The high number of reference images makes the structures of the disk very distinct within the cube enriched with the references, so they are not captured as the main components. We can, therefore, use a higher rank to capture more star structures. To increase the number of references without having to duplicate frames, we have selected, from among all the reference stars, those that are most correlated (with PCC). Note that, if there were a few more degrees of rotation, such as the spots of a FHWM-size that compose the speckle field would not be considered flux invariant to the rotation, considering the definition given in \citet{Sandrine}, as is the case in some star hopping games, the quality of the results would probably be much better. 
\end{enumerate}



\begin{figure}[!t]
        \centering
         \includegraphics[width=\linewidth]{Images/Planetflux.png}
        \caption{Measurement of the planet flux compared to the ground truth in disk \#E at contrasts of $10^{-3}$ and $10^{-4}$. The two columns of this plot represent the same tests as the two last columns (disk \#E) of the two first tables (contrasts $10^{-3}$ and $10^{-4}$) displayed in Figure \ref{fig:results}. The three bar plots in each cells compare the flux measurements of RDI/PCA, ADI/IPCA, and ARDI/IPCA. The displayed values correspond to the ratio in percentage of the estimated flux in a FHWM-aperture located at the planet position over the ground truth. The cell background is colored according to the strategy achieving the closest value of flux to the ground truth. When no PLF was observed at the planet location, the bar plots are replaced by the text 'N/D' to indicate non-detection.}
        \label{fig:planetflux}
\end{figure}

\item In terms of the restoration of the planet in disk \#E, as observed in Figure~\ref{fig:planetflux}, we note that the measured flux of the planet tends to be systematically underestimated by the three algorithms. At a contrast of $10^{-3}$, the planet is detected within the disk by all three strategies. ARDI recovered the flux better than the two other strategies three out of four times, achieving a recovery of 79.2\% of the planet flux on average and remaining consistent across all tests. In comparison, RDI recovers 72.2\% of the planet flux on average, but its correctness varies from 102\% to 57\%. ADI underperforms compared to the two other strategies, with only 57\% of the planet flux recovered on average. At a contrast of $10^{-4}$, the planet is systematically detected with ADI but never detected with RDI. In fact, at a higher contrast, RDI struggled to capture the planet, while ADI had difficulty capturing the disk structure. ARDI captures both the planet and the disk structure for cubes \#2, \#3, and \#4 but fails to recover either the disk or the planet for cube \#1. In terms of flux recovery, neither ARDI nor ADI seems to stand out. Either the flux appears to be significantly underestimated, which also coincides with the image lacking disk structure, or the flux is overestimated due to artifacts arising at a small separation from the star near the planet.
